Surfacing Visualization Mirages

Dirty data and deceptive design practices can undermine, invert, or invalidate the purported messages of charts and graphs. These failures can arise silently: a conclusion derived from a particular visualization may look plausible unless the analyst looks closer and discovers an issue with the backing data, visual specification, or their own assumptions. We term such silent but significant failures "visualization mirages". We describe a conceptual model of mirages and show how they can be generated at every stage of the visual analytics process. We adapt a methodology from software testing, "metamorphic testing", as a way of automatically surfacing potential mirages at the visual encoding stage of analysis through modifications to the underlying data and chart specification. We show that metamorphic testing can reliably identify mirages across a variety of chart types with relatively little prior knowledge of the data or the domain.

==> pipeline.tex <==
\section{A Mirage Generation Pipeline}


\begin{figure*}[t]
   \centering
   \includegraphics[width=2\columnwidth]{mirages.pdf}
   \caption{
   Each stage in the visual analytics process offers users agency but also presents an opportunity for errors, which can give way to mirages.
   %Visualization mirages can come from all points of action in the visualization pipeline. 
   We attempt to identify the dependencies between actions, errors they create, and ways that those errors can propagate to deceive the reader.
   %We use colored blocks throughout the paper to indicate issues that can arise during the Curation \CURATING, Wrangling \WRANGLING, Visualizing \VISUALIZING, and Reading \READING of data.
   }
   \label{fig:mirage-figure}
\end{figure*}

We delineate how choices can create errors and highlight the way that those errors can propagate to become mirages in \figref{fig:mirage-figure}. 
We focus on moments of agency in the visual analytic process (denoted in our diagram by arrows) that can introduce failures either by themselves, or in concert with other decisions, to generate visualization mirages. 
% am: this sentence is clumsy, the start is poorly phrased and the end is not yet setup (see above todo about automated systems)
This perspective gives us clues as to the casual relationship between choices and mirages, which is beneficial to our larger goal of being able to automatically surface these issues to the chart creator. 
%Our model builds pipeline such as those in Borland \etals \cite{borland2018contextual} for where threats to validity arise in analytics, Sacha \etals~\cite{sacha2015role} model of how visualization awareness and trust disseminate, as well as Heer's \cite{heer2019Visualization} description of points of failure in the analysis process.
Our model builds upon pipeline-based descriptions of problems in the visual analysis process. Our work most notably expands upon Borland \etals \cite{borland2018contextual} categorization of where threats to validity arise in visual analytics, Sacha \etals~\cite{sacha2015role} model of how visualization awareness and trust disseminate across the sensemaking loops of the process, and Heer's \cite{heer2019Visualization} description of the points of failure across the acts of analysis.


Consider a concrete example: the bar chart in \figref{fig:deception-quartet} purports to show that average sales for Y are higher than for X. However, there are many potential data sets that could produce that final chart, many of which would cause a reasonable person to doubt the conclusion that sales for Y are higher in a meaningful or predictive sense. For instance, the difference could be driven by a single outlier (B). Or the difference could be driven by one value repeated dozens of times (C). Or through a severe mismatch in the number of records aggregated to produce the final value (D). These potential data quality issues are invisible in the final aggregate bar chart (just as many other significant differences are hidden through summarization or aggregation~\cite{anscombe1973graphs, matejka2017same}), and some may only be visible in more complex visualizations like dot plots with appropriate design parameters.  

%An important component of a mirage is the purported (misleading, fragile, or hallucinatory) message that is being communicated in the visualization. The nature of this message is dependent on the reader and the reader's task. What may be misleading in the context of one task may not interfere with another: for instance, bias in estimating angle caused by a poorly selected aspect ratio~\cite{heer2006multi} or improperly selected scales~\cite{cleveland1982variables} could potentially produce a mirage for a viewer interested in correlation, but is unlikely to impact a viewer interested in locating extrema.
% TASK PARAGRAPH



\subsection{A Model of Visual Analytics for Exposing Mirages}
% \am{I think the start of this section (fast tour of model components) can be compressed pretty hard, as it stands it's somewhat content-free.}

\am{INTRO SENTENCE}
Our model begins with the origins of the data. Following prior scholarship~\cite{gitelman2013raw,dignazio2019draft,dork2013critical,haraway1988situated}, we do not credit the notion of \emph{raw data} that arises from objective observation, but rather argue that the structure, sources, and perspectives of people shape the nature of the data. 
Choices of how to navigate our situated environment to produce data can therefore induce mirages or deceptions. We use the term \textbf{Curating}\CURATING{ }to denote this entire process of measuring, organizing, combining, and collecting data.
%As Onuoha puts it: \textit{``Data sets are the results of their means of collection''}\cite{onuoha2016Point}, a degree of analyst agency which can cause there missing datasets or malformed inputs that warp the rest of the analysis in a manner that is often invisible.
%
Once the datasets are created, the analyst must clean, filter, subset, model, and shape the data into a form that is usable by the visualization system. We refer to this step as \textbf{Wrangling}\WRANGLING. 
% 
This stage offers the analyst a large number of ``researcher degrees of freedom''~\cite{gelman2013garden} which can lead to irregularities and false-positives in their work. A larger discussion of this relationship between statistical malpractice, or other questionable research practices, and visualization can be found elsewhere \cite{huff1993lie, pu2018garden, dragicevic2019increasing}, our focus is primarily on the types of defenses that prior work has employed against these problems.
%The inclusion of modeling and subsetting under this step includes many of the ``researcher degrees of freedom''~\cite{gelman2013garden} that can lead to irregularities and false-positives in scientific work. A full accounting of statistical malpractice or other Questionable Research Practices is out of the scope of this paper (but see e.g. Huff~\cite{huff1993lie}, Pu \& Kay~\cite{pu2018garden}, or Dragicevic \etal~\cite{dragicevic2019increasing} for how these issues can arise in visualization). 
%
Once the data are in a proper form, the next step is to render the data in some human-legible way. We refer to this step as \textbf{Visualizing}\VISUALIZING. 
%Many potential designs in this category are not literally charts, such as tables or natural language summaries.
\am{HOW CAN THIS STUFF GO WRONG??}
%
The last step is then for a human to read, interpret, and comprehend the resulting design. This \textbf{Reading}\READING{ } involves the literal decoding of the visual variables in a chart to retrieve the values of interest, as well as reasoning about the importance of the patterns identified in the data and updating prior beliefs based on new information.%, or persuading audiences of a particular data-driven position. AM: third clause changes user type
\am{HOW CAN THIS STUFF GO WRONG??}
%
%Woohoo, time for a ToC paragraph!
%\am{We don't really describe that many vectors of attack in the following sections so it might be best to drop this metaphor? That or we should actually describe stuff that can go wrong. AM UPDATE: i'm workin on it}
In the following sections, we explore how mirages can arise from choices at many stages of the visualization pipeline lensed and grouped through already known topics in the literature. To borrow a metaphor from security, we investigate the ``vectors'' that make up our ``attack surface.'' In addition to attacks, we also focus on defense: we investigate methods for detecting errors or bad practices in either a mixed-initiative~\cite{horvitz1999principles} or fully automatic way. 

%I know I said we needed a forward pointer here, but I wonder if it goes to the end of this full section as a transition sentence, rather than here.

%Once these attack surfaces are established we will describe a novel technique for defending against a subset of these vectors \VISUALIZING\READING by combining previous work on linting for visualization with notion of metamorphic testing (or automated perturbative input testing) from software engineering.


\begin{figure}[bth]
   \centering
   \includegraphics[width=\columnwidth]{misspelling-bar-charts.pdf}
   \caption{
   Mirages can be caused by data curation errors \CURATING, such as in this synthetic example in which a spelling mistake in the curation process causes a grouping error, which in turn causes an inaccurate inference about the data.
   }
   \label{fig:misspelling}
\end{figure}

\begin{figure}[bth]
   \centering
   \includegraphics[width=\columnwidth]{wrangling-error.pdf}
   \caption{
   The level of aggregation in this graph obscures missing data (in this case, missing data for all of the fall months of 2010). This wrangling error \WRANGLING{ }gives the false impression that sales were significantly down during fall of 2010.
   }
   \label{fig:wrangling}
\end{figure}


\subsubsection{\CURATING\WRANGLING{ }Dirty Data}

The efficacy of a visualization is limited by the quality and characteristics of its backing data. Even the most well-designed chart will be fundamentally flawed if the data on which it relies is irrelevant, incomplete, or biased \CURATING, or has been process in an uncareful or error producing manner \WRANGLING.
%
In tandem these types of issues are typically referred to as \emph{dirty data} (see Kim \etals~\cite{kim2003taxonomy} useful taxonomy of dirty data for extensive discussion).
A simple example of the negative effect that dirty data, or its mishandling, can lead to mirages can be seen in \figref{fig:misspelling}.
% this idea/sentence pair needs to be reoraganized
%Kim \etal~\cite{kim2003taxonomy} present a taxonomy of issues that can create ``dirty data.'' Many of these issues can also result in visualization mirages.  
Tang \etal~\cite{tang2019towards} describe the challenge of automatically detecting and understanding the ways in which dirty data can creating misleading trends as one of the most important open problems in visualization.
%
\figref{fig:deception-quartet} presents three examples: errors in data prep can result in outliers, repeated values, or missing values, creating changes in the resulting visualizations of the data that may or may not represent genuine patterns of interest. \am{TODO list some more mirages at this step}


% The process of cleaning a dataset is an expensive process (in time, complexity, and effort) involving expertise. In a 2016 Crowdflower survey, data scientists reported that the majority of their time was spent collecting and cleaning datasets~\cite{forbesdata}. % am: i don't think this citation is relevant in it's current phrasing

There are a number of different approaches for automatically defending against data quality issues. Most relevant to our approach, Mu\c{s}lu \etal~\cite{mucslu2015preventing} employ the metaphor of continuous testing to detect potential data quality concerns and Hynes \etal~\cite{hynes2017data} propose a data ``linter'' and find that many common datasets for use in training and evaluating machine learning models contain elementary data quality issues. 
%
Wang and He~\cite{wang2019uni} propose an automated error detection system for tables based on statistical analyses. 
%
Barowy \etal present systems both for ``data debugging'' in spreadsheets~\cite{barowy2014checkcell} and spreadsheet formulae~\cite{barowy2018excelint}. 
%
Many systems employ combinations of statistical algorithms, visualizations, and manual inspection to detect and correct data quality issues~\cite{kandel2011research}. This mixed-initiative data wrangling metaphor is instantiated in  systems such as Potter's Wheel~\cite{raman2001potter}, Profiler~\cite{kandel2012profiler}, and Data Tamer~\cite{stonebraker2013data}, as well as in commercial solutions like Tableau Prep and Trifacta \am{do these need citations?}.



\begin{figure}[bth]
   \centering
   \includegraphics[width=\columnwidth]{radars.pdf}
   \caption{
    Radar charts are often used to compare the skills of individuals in sports and job hunting \protect\cite{filipov2019cv3}. Here we show two radars of the programming language skills for a hypothetical job candidate. One axis ordering seems to suggest that candidate is skilled in one area, while the other suggests that their skills are varied. Both of these interpretations hallucinate meaning that is not actually present in the data, an example of an AVD Hallucinator \protect\cite{kindlmann2014algebraic}.}
   \label{fig:radarsz}
\end{figure}



\subsubsection{\WRANGLING\VISUALIZING{ }Volatile Visualizations}
%\mc{TODO: AVD example image}
%\mc{AVD diagram goes here, perhaps just with $\alpha$ and $\omega$-related errors (labeled with orange and red squares?}
\am{Volatile visualization contain avd no?}
Kindlmann \& Scheidegger~\cite{kindlmann2014algebraic} point to a class of visualization failures that follow from violations of the ``Algebraic Visualization Design'' framework. Under the AVD framework, trivial changes to the data (such as shuffling the row order of input data) should result in trivial changes in the resulting visualization, and important changes in the visual appearance of the visualization should only occur as a result of important changes in the backing data. Failures of these assertions can result in ``hallucinators'' (visualizations that look dramatically different despite being backed by similar or identical data, such as in \figref{fig:radarsz}) and ``confusers'' (visualizations that look identical despite being backed by dramatically different data). In the worst case, visualizations can be completely non-responsive to their backing data, functioning as mere number decorations and creating what Correll \& Heer~\cite{correll2017black} refer to as visualization ``non-sequiturs.''

\am{TODO:  integrate hibbard lattices \cite{hibbard1994lattice} and jock's \cite{mackinlay1986automating}}

The inability of visualization designs to respond correctly to important changes in the underlying data, or to exaggerate trivial changes, is under-explored. Rogowitz~\cite{rogowitz2001blair,rogowitz1996not} explore how minor alternations to color maps can result in different perceptions of patterns in visualizations. Also relevant to our work is the use of ``graphical inference''~\cite{wickham2010graphical} where viewers look at multiple visualizations generated under some null hypothesis and one visualization of the actual data, and must identity the ``guilty'' visualization showing the pattern of interest amongst the ``innocent'' null visualizations. Hofmann \etal~\cite{hofmann2012graphical} use reliability at performing this task as a proxy for the statistical power of a visualization~\cite{hofmann2012graphical}; Correll \etal~\cite{correll2018looks} specifically use graphical inference to diagnose algebraic visualization design concerns. Visualizations where graphical inference is unreliable suggest that either the statistical pattern of interest is not robust or that the visualization design employed is insensitive to such patterns.

A related issue to AVD is the notion of statistical robustness and reliability; visualizations should ideally not promote interpretations of the data that are accidents of sampling error or generally not well-supported by the backing data. Pu \& Kay~\cite{pu2018garden} caution that visual analytics systems that allow arbitrary amounts of filtering, drill-down, and sampling, can function as ``p-hacking machines'' that generate spurious conclusions. Zgraggen \etal~\cite{zgraggen2018investigating} found that, in systems without visualizations of statistical uncertainty or control for robustness, many if not most of ``insights'' reported from a sample of a dataset failed to be true of the larger dataset. Other issues that occur through the process of visual exploration of dataset are Simpson's paradox~\cite{armstrong2014visualizing,guo2017you} (where patterns in data appear to reverse based on the level of categorical aggregation and the relative sample size) and the drill-down fallacy~\cite{lee2019avoiding} (where ignoring explanatory variables during the process of filtering can result in erroneous claims of causality).

Proposed mixed-initiative solutions to issues of robustness involve supplementing visualizations with additional metrics that indicate their reliability~\cite{binnig2017toward,zhao2017controlling}, or performing pre-analyses to automatically detect potential concerns in a dataset~\cite{guo2017you}. Veras \& Collins see robustness as a matter of visualization scalability and deploy a metric-based approach to identify visualization that don't reliably reflect their data \cite{veras2019discriminability}. Lunzer \& McNamara also explore the robustness of a visualization by superimposing alternative chart configurations on top of one another \cite{lunzer2014aint}.


\begin{figure}[bth]
   \centering
   \includegraphics[width=\columnwidth]{mens-run.pdf}
    
   \caption{
%  \mc{Example figure of a design producing an perfectly grammatical visualization that is nonetheless deceptive. Perhaps Huff style ``gee whiz'' graph? (teal square)}
 Changes to Men's 100-meter dash world record over the last century. The left image suggests that there hasn't been much change in that time, yet the image on the right tells a more evocative story. This demonstrates how visualizations can be grammatical yet deceptive \READING. 
% \am{I'm not sure this is a good example, would love commentary}
   }
   \label{fig:deceptive-axes}
\end{figure}

\subsubsection{\VISUALIZING\READING{ }Deceptive Designs}
The potential harm in the uncritical consumption, or malicious design of visualizations is well-known. Bresciani \& Eppler~\cite{bresciani2009risks,bresciani2015pitfalls} enumerate various ``risks'' and ``pitfalls'' that can occur when interpreting visualizations. Huff~\cite{huff1993lie} presents many examples of misleading charts in \emph{How to Lie With Statistics} and Wainer~\cite{wainer1984display} likewise presents a guide on ``how to display data badly,'' and Szafir \etal~\cite{szafir2018good} enumerate ``five ways that visualizations can mislead.'' More recently, Correll~\cite{correll2017black} enumerates a class of visualization ``attacks'' that do not misrepresent the data \emph{per se} but may still mislead the viewer, and Cairo has explored numerous ways that charts can ``lie''~\cite{cairo2015graphics,cairo2019}. \am{TODO ref \figref{fig:deceptive-axes}}

Prior work in visualization has found that deceptive practices can have measurable deleterious impacts on the comprehension of charts. Pandey \etal~\cite{pandey2015deceptive} find that commonly discussed errors such as truncated y-axes and size/area confounds impact subjectively assessed trends and differences in values. Kong \etal~\cite{kong2018frames,kong2019trust} find that slanted and biased chart titles can impact how the data are later recalled. Cleveland \etal~\cite{cleveland1982variables} find that scale alterations can bias the perception of correlation in scatterplots, and Newman \& Scholl~\cite{newman2012bar} find that bar charts create a bias when viewers estimate the likelihood of samples. While avoiding known practices is often instantiated in the defaults or guidelines of visualization authoring systems (such as Draco~\cite{moritz2018formalizing}), to our knowledge no system exists that automatically detects or surfaces deceptive elements of a visualization design.

Even if the visualization designs are not deceptive, our cognitive biases can still cause us to come away with incorrect or unjustified assumptions about the data~\cite{dimara2018task}. Similar to our work, Wall \etal~\cite{wall2017warning} propose a system that automatically augments a visual analytics system with warnings about cognitive biases that may be present in the current course of analysis. 

\begin{figure}[bth]
   \centering
\subfloat[Crime shown by Trulia~\protect\cite{trulia}]{\includegraphics[width=.45\linewidth]{missing-dataset-trulia.png}}\qquad
\subfloat[White collar crime \protect\cite{lavigne2017predicting}]{\includegraphics[width=.45\linewidth]{missing-dataset-white-collar.png}}
   \caption{Crime maps typically are generated by 911 calls and police reports, which capture only a subset of criminal activity focused on violent crime. In contrast, white collar crimes are often excluded from these maps, presenting a biased message of the relative criminality of different regions that is linked to socio-economic status rather than personal or economic danger.
   %Lavigne \etals map of white collar crime provides a commentary on this matter \protect\cite{lavigne2017predicting}, here juxtaposed with a neighborhood safety map published by online-realtor Trulia \protect\cite{trulia}. \am{REDO this caption for clarity if it's to be kept in}
   }
   \label{fig:missing-datasets}
\end{figure}


\subsubsection{\READING\CURATING{ }Uncritical Charts}
% \am{Maybe should include some commentary on how this is different than the previous section?}
%\mc{Still don't like this title (not least of which because it's not a consonance like the other two sections. Possible other options: Valueless Visualizations, Virtueless Visualizations, ...}
%\am {i think i still like uncritical best}
%\am{Right Problem Wrong Dataset: Generate a figure showing a visualization that appears to be correct, but in fact the backing data that has been selected is totally inappropriate for that problem, needs to be somewhat realistic in order to make a convincing sell. 
%
%MCs suggestion of using either White Collar Crimes or Trump Islands?
%An uninteresting idea: asking what the weather in san francisco may seem like a simple question, at 7x7 miles it is a rather small city after all, yet the true answer is not so simple. An analyst trying to determine a buisness quantity like number of "hot" days in the city might consider a city wide average, yet because of its extremely heterogenous topography that number might not be accurate for a huge number of neighborhoods within the city.
%}


Reading errors\READING can occur in conjunction with other parts of the pipeline, such as with Curating errors\CURATING.
%In addition to uncritical comprehension of visual information, visualizations are vulnerable to uncritical construction. 
% When engaging in the chart-making process the chart designer may not appropriately communicate their biases and assumptions about the data, their audiences bias and assumptions about the data, or the structures of power latent in the communication therein. 
Chart makers may not appropriately communicate their biases and assumptions about the data or they might not predicate how their audiences bias and assumptions about the data may affect the reading of the image. 
%
Without appropriate context, readers often believe charts present an objective view-from-nowhere~\cite{haraway1988situated}, as opposed to its inherently persuasive and subjective role.
%\mc{Quibble, but ``accounting for biases'' still suggests a sort of view from nowhere.}
%
A visualization may address the right problem but be doing so using the wrong data set or there may be a mismatch between assumptions about the data and the data itself, as in \figref{fig:missing-datasets}.
%
Beyond errors in data entry or federation, there are questions of who is or is not included in particular datasets. Who counts, and who is counted in a dataset can have a great deal of impact in the resulting conclusions drawn from it~\cite{dignazio2019draft, correll2019ethical}.
%
Peck \etal consider the consequences of a related issue: who is assumed to be reading a visualization? They conclude that a visualization's effectiveness can be marred by excluding the ``data poor" from the assumed audience for that visualization \cite{peck2019data}--- those without the statistical or graphical literacies to make good use of the visualizations they receive.
%
If analyst were trying to the rate of unemployment in United States, they  might count the number of unemployed workers over the total labor force. This number would be intrinsically incorrect: as it would not incorporate currently incarcerated individuals, as statistics for that population do not exist \cite{missingdatasets}.
%
\am{DESCRIBE MORE ATTACKS}



Defenses in this regime often focus on providing tools for introspection that help identify bias and perceptual problems.
%
D{\"o}rk \etal \cite{dork2013critical} describe a four point system for critically analyzing infographics. Lupi articulates a manifesto of ways for chart makers to reconsider their relationship with their data and render image \cite{lupi2017data}, such as valuing subjective data.  Wood \etal ask visualization designers to engage with potential problems originating at different stages in the design process through linted design-schemas \cite{wood2018design}, which ask designers to answer questions from a variety of sources including D'Ignazio \& Klein's Feminist Data Visualization \cite{d2016feminist} such as ``How do I communicate the limits of my categories in the final representation?"
%
A persistent line of advice (and here defence against threats to ecological validity) in visualization emphasizes data-ink minimalism \cite{tuftevisualdisplay}, which pushes designers to assume that their reader will be distracted and confused by chart embellishments and decorations. A number of authors critique this position, noting minimal charts do not facilitate memorability \cite{bateman2010useful}, or engagement \cite{hullman2011benefitting}. In tandem this can cause readers to ignore or forget a charts message: a mirage in time. % AM: could also cite: correll2014badoh h 
%
In related critiques, Kostelnick points to the ``conundrum of clarity''~\cite{kostelnick2008visual} as a way of hiding the rhetorical power of visualizations, and Dragga \& Voss~\cite{dragga2001cruel} suggest that using the same unadorned style for visualizations of dramatically different ethical importance is ``cruel.''
%However a number of works critique this position, which seems to forget that there are people reading this graphics.
%However, Bateman \etal posit that emotionally evocative chart decorations (such as the famous monstrous bar chart) increase the memorability of charts \cite{bateman2010useful}. Hullman \etal similarily posit that visualizations that are more difficult, or visually complex, can cause the reader to spend more time with the work and hence better appreciate its message \cite{hullman2011benefitting}. 
%
%\am{maybe include a pointer to deno?, doing so would also necessitate pointing at mulching proposal}
%AM: MAYBE CITE THAT BIAS TAXONOMY.


\section{Using Our Model}

We treat the creation of visualization mirages as a mistake, error, or intentional deception that occurs somewhere along the pipeline in ~\figref{fig:mirage-figure}. Note that the mirage need not occur directly after the point of failure: a mirage might only occur if an error upstream is not ``caught'' by decisions downstream. For instance, values that were erroneously repeated when creating a dataset might create a mirage if the data are visualized in an aggregated bar chart, but an alternative visual design, such as a dot plot, would reveal the abnormality, dispelling the mirage.
%
We enumerate a collection of potential generators of visualization mirages in Table \ref{table:mirage-table}, colored and grouped based on which action in our flow diagram creates the mirage. This list is by no means complete; a full categorization of all the ways that we can deceive or mislead with data is out of the scope of this work. We focus in this table on particularly powerful examples of mirage generators, with a secondary focus on issues that propagate \emph{along} our pipeline, rather than just at one stage of the process. 
\am{TODO: need some discussion of uh using our model or how wt think it might be used}

%Where possible, we consult existing surveys of error types. For instance for errors in data entry \CURATING\WRANGLING we consult a survey by Kim \etal~\cite{kim2003taxonomy}, and for errors in visualization design and comprehension \VISUALIZING\READING we draw from visualization pitfalls identified by Bresciani \& Eppler~\cite{bresciani2015pitfalls} and cognitive bias in visualization analytics by Dimara \etal~\cite{dimara2018task}. A longer version of this table is available in the supplementary materials.
%In addition to synthesizing these multiple sources into a complete whole, our approach also informs the design of our tool, \SYSTEMNAME, which specifically tests for mirages by combining both a direct consultation against specific issues but also a more generalized approach that checks for robustness and reliability by altering one or more steps along our pipeline and checking the resulting final visualization for important differences.

\input{mirage-error-table.tex}

